Spectral Rewiring for Exploration, Purification, and Model Merging

Reinforcement learning has become a standard post-training recipe for large language models, but dense full-parameter updates create two deployment-relevant bottlenecks: suppressed reasoning performance, often reflected by premature saturation of test-time scaling, and interference when consolidating multiple capabilities through multi-domain training or model merging. We show that the reasoning-effective component of these updates is largely concentrated in the base model's spectral space, motivating Subspace-Aligned Rewiring (SAR), a post-hoc editing method that retains this spectral core while removing orthogonal components. SAR therefore preserves reasoning gains and filters residual update directions that suppress performance or amplify cross-domain interference. Across several model families and scales, SAR extracts compact reasoning cores using as little as approximately 0.58% of total parameters: it preserves over 99% of post-training performance and improves high-k exploration in mathematical reasoning, and generalizes to agentic coding by improving six of seven open benchmarks on an in-house model. SAR also purifies mixed-domain training updates by releasing suppressed coding capability while maintaining math reasoning and instruction following. It further enables model merging across experts, yielding cross-domain generalization that surpasses previous merging baselines and even the best single-domain experts. Overall, SAR shows that extracting reasoning-effective updates from parameter geometry can serve as a training-free mechanism to improve reasoning and multi-domain performance.

==> sections/contributions.tex <==
\newpage
\section*{Contributions}

\textbf{Project Lead}\quad 

Author A$^{1,2}$


\textbf{Algorithm}

Author A$^{1,2}$, Author B$^{2}$

\textbf{Infrastructure$^{*}$}

Author A$^{1,2}$, Author B$^{2}$, Author C$^{1,2}$

% $^{*}$Last-Name in Alphabetical Order

\textbf{Dataset}

Author B$^{2}$

\textbf{Supervision}

Author C$^{1,2}$


\textbf{Affiliation}

$^1$Generative Symbolic Intelligence Lab (GenSI), Tsinghua University 

$^2$Institute for AI Industry Research (AIR), Tsinghua University

\section*{Acknowledgments}

We thank xxx for xxx
